Beyond GWTC-3: Analysing and verifying new gravitational-wave events from community catalogues

The public release of data from the LIGO and Virgo detectors has enabled the identification of potential gravitational wave signals by independent teams using alternative methodologies. In addition to the LIGO-Virgo-KAGRA (LVK) collaboration's GWTC-3 catalogue there have been several additional works claiming the detection of signals in the data from the first three observing runs. In this paper we present an analysis of these new signals using the same analysis workflow which was used to generate the GWTC-2.1 and GWTC-3 catalogues published by the LVK, matching the analysis configuration as closely as possible, and we provide our parameter estimation results in a format comparable to those of the GWTC-3 data release. We also include a discussion of the workflow developed for this analysis.

==> divergence-macros-o3a.tex <==
\DeclareRobustCommand{\chirpmasssourcethreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\massratiothreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chieffthreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chipthreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\luminositydistancethreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chirpmasssourceIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.83}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\massratioIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.20}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chieffIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.22}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chipIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.12}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\luminositydistanceIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.07}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}


==> figures/divergence-macros-o3a.tex <==
\DeclareRobustCommand{\chirpmasssourcethreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\massratiothreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chieffthreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chipthreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\luminositydistancethreeOGCdivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{--}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chirpmasssourceIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.83}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\massratioIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.20}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chieffIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.22}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\chipIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.12}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}
\DeclareRobustCommand{\luminositydistanceIASthreedivergence}[1]{\IfEqCase{#1}{{GW190426_082124}{--}{GW190427_180650}{--}{GW190511_125545}{--}{GW190511_163209}{--}{GW190514_065416}{--}{GW190523_085933}{--}{GW190530_030659}{--}{GW190530_133833}{--}{GW190604_103812}{--}{GW190605_025957}{--}{GW190607_083827}{--}{GW190614_134749}{--}{GW190615_030234}{--}{GW190705_164632}{--}{GW190707_083226}{--}{GW190711_030756}{--}{GW190718_160159}{--}{GW190725_174728}{--}{GW190805_105432}{--}{GW190806_033721}{--}{GW190814_192009}{--}{GW190818_232544}{--}{GW190821_124821}{0.07}{GW190906_054335}{--}{GW190910_012619}{--}{GW190911_195101}{--}{GW190916_200658}{--}{GW190920_113516}{--}{GW190926_050336}{--}}}

